In-Context Freeze-Thaw Bayesian Optimization for Hyperparameter Optimization

With the increasing computational costs associated with deep learning, automated hyperparameter optimization methods, strongly relying on black-box Bayesian optimization (BO), face limitations. Freeze-thaw BO offers a promising grey-box alternative, strategically allocating scarce resources incrementally to different configurations. However, the frequent surrogate model updates inherent to this approach pose challenges for existing methods, requiring retraining or fine-tuning their neural network surrogates online, introducing overhead, instability, and hyper-hyperparameters. In this work, we propose FT-PFN, a novel surrogate for Freeze-thaw style BO. FT-PFN is a prior-data fitted network (PFN) that leverages the transformers' in-context learning ability to efficiently and reliably do Bayesian learning curve extrapolation in a single forward pass. Our empirical analysis across three benchmark suites shows that the predictions made by FT-PFN are more accurate and 10-100 times faster than those of the deep Gaussian process and deep ensemble surrogates used in previous work. Furthermore, we show that, when combined with our novel acquisition mechanism (MFPI-random), the resulting in-context freeze-thaw BO method (ifBO), yields new state-of-the-art performance in the same three families of deep learning HPO benchmarks considered in prior work.

==> icml2023/latex/algo.tex <==
\begin{algorithm}
\small
  \caption{Freeze-thaw vs. Black box BO \label{algo:ftbo}}
  Contrasts the online learning (\textcolor{green}{\olftbo}), our in-context learning Freeze-thaw (\textcolor{blue}{\ours}), and black box (\textcolor{red}{\bbbo{}}) approaches to Bayesian optimization for HPO. Code specific to these methods is shown in \textcolor{green}{green}, \textcolor{blue}{blue}, and \textcolor{red}{red}, respectively. Code shared by all methods is shown in black, code shared between both \textcolor{teal}{\ftbo{}} variants in \textcolor{teal}{blue green}, and code shared between \bbbo{} and \olftbo{} (\textcolor{brown}{not \ours}) in \textcolor{brown}{brown} \\
  \textbf{Input:} The configuration space $\Lambda$ \\
  \textbf{Input:} The measure of model performance $f$ to be minimized \\
  \textbf{Input:} The maximal training run length $b_{max}$ in training steps \\
  \textbf{Input:} The total HPO budget $B$ in training steps \\
  \textbf{Component:} The \textcolor{teal}{dynamic} surrogate model $g$ \\
  \textbf{Component:} The \textcolor{teal}{dynamic} acquisition function $a$ \\
  \textbf{Output:} The configuration $\lambda \in \Lambda$ obtaining the best model \\
  \textbf{Procedure} HPO($\Lambda$, $f$, $b_{max}$, $B$):
  \begin{algorithmic}
      \STATE $\lambda \sim \mathcal{U}(\Lambda)$
      \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
      \STATE \textcolor{teal}{$H = \{(\lambda, 1, f(\lambda,1))\} \gets {\sc evaluateFT}(\lambda)$}
      \WHILE{$|H| < B$}
        \STATE \textcolor{brown}{g.fit(H)} \textcolor{blue}{\COMMENT{\ours{} does not require refitting the PFN}}
        \STATE $\Lambda' = \{\lambda\}_{\lambda \in \Lambda:\, (\lambda, b_{max}, \cdot) \notin H}$
        \STATE \textcolor{red}{$P = \{\lambda,\,g(\lambda)\}_{\lambda \in \Lambda'}$}
        \STATE \textcolor{teal}{$P = \{\lambda,t,\,g(\lambda,t\textcolor{blue}{,H})\}_{\lambda \in \Lambda',\, t > b_\lambda}$}
        \STATE $\lambda = \argmax_{\lambda \in \Lambda'} a(P)$
        \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
        \STATE \textcolor{teal}{$H = \{(\lambda, b_\lambda+1, f(\lambda,b_\lambda+1))\} \gets {\sc evaluateFT}(\lambda)$}
    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,t)\}_{(\lambda, t, f(\lambda,t)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}

==> icml2023/latex/algo_new.tex <==
\begin{algorithm}
\small
  \caption{Freeze-thaw vs. Black box BO \label{algo:ftbo}}
  Contrasts the online learning (\textcolor{green}{\olftbo}), our in-context learning Freeze-thaw (\textcolor{blue}{\ours}), and black box (\textcolor{red}{\bbbo{}}) approaches to Bayesian optimization for HPO. Code specific to these methods is shown in \textcolor{green}{green}, \textcolor{blue}{blue}, and \textcolor{red}{red}, respectively. Code shared by all methods is shown in black, code shared between both \textcolor{teal}{\ftbo{}} variants in \textcolor{teal}{blue green}, and code shared between \bbbo{} and \olftbo{} (\textcolor{brown}{not \ours}) in \textcolor{brown}{brown} \\
  \textbf{Input:} configuration space $\Lambda$, measure of model performance $f$ to be minimized, maximal training run length $b_{max}$ in training steps, total HPO budget $B$ in training steps \\
  \textbf{Component:} \textcolor{teal}{dynamic} surrogate model $g$ and \textcolor{teal}{dynamic} acquisition function $a$ \\
  \textbf{Output:} the configuration $\lambda \in \Lambda$ obtaining the best model \\
  \textbf{Procedure} \textsc{HPO}($\Lambda$, $f$, $b_{max}$, $B$):
  \begin{algorithmic}
      \STATE $\lambda \sim \mathcal{U}(\Lambda)$
      \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
      \STATE \textcolor{teal}{$H = \{(\lambda, 1, f(\lambda,1))\} \gets {\sc evaluateFT}(\lambda)$}
      \WHILE{$|H| < B$}
        \STATE \textcolor{brown}{g.fit(H)} \textcolor{blue}{\COMMENT{\ours{} does not require refitting the PFN}}
        \STATE $\Lambda' = \{\lambda\}_{\lambda \in \Lambda:\, (\lambda, b_{max}, \cdot) \notin H}$
        \STATE \textcolor{red}{$P = \{\lambda,\,g(\lambda)\}_{\lambda \in \Lambda'}$}
        \STATE \textcolor{teal}{$P = \{\lambda,t,\,g(\lambda,t\textcolor{blue}{,H})\}_{\lambda \in \Lambda',\, t > b_\lambda}$}
        \STATE $\lambda = \argmax_{\lambda \in \Lambda'} a(P)$
        \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
        \STATE \textcolor{teal}{$H = \{(\lambda, b_\lambda+1, f(\lambda,b_\lambda+1))\} \gets {\sc evaluateFT}(\lambda)$}
    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,t)\}_{(\lambda, t, f(\lambda,t)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}

==> icml2023/latex/algo_rebu-copy.tex <==
\begin{algorithm}
  \small
  \caption{Freeze-thaw BO \label{algo:rebuttal-ftbo-copy}}
  \textbf{Input:} 
    configuration space $\Lambda$, \\
    \textbf{Output:} $\lambda \in \Lambda$, obtaining the best performance \\
  \textbf{Procedure:} HPO($\Lambda$, $f$, $\mathds{1}_b$, $b_{max}$, $B$): \\
  \begin{algorithmic}
      \STATE $\hat{f}\rightarrow{}$initialize surrogate modelp)
      \WHILE{$|H| < B$}
     \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}~~~$\rhd$~no model fitting in FT-PFN
    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,b)\}_{(\lambda, b, f(\lambda,b)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}



==> icml2023/latex/algo_rebu.tex <==
\begin{algorithm}

\small
  \caption{Freeze-thaw BO \label{algo:rebuttal-ftbo}}
  \textbf{Input:} 
    configuration space $\Lambda$, \\
    measure of model performance $f$ to be minimized, \\
    value of unit step budget $\mathds{1}_b$,~~~$\rhd$~epoch(s)/update(s)\\
    maximal steps $b_{max}$, ($\forall~\lambda \in \Lambda$)\\
    total HPO budget $B$ in training steps \\ 
    
    \textbf{Output:} $\lambda \in \Lambda$, obtaining the best performance \\
    
  \textbf{Procedure:} HPO($\Lambda$, $f$, $\mathds{1}_b$, $b_{max}$, $B$): \\
  \begin{algorithmic}
      \STATE $\hat{f}\rightarrow{}$initialize surrogate model
      \STATE $\lambda \sim \mathcal{U}(\Lambda)$~~~$\rhd$~initial random sample
      \STATE $H \leftarrow{} \{(\lambda, \mathds{1}_b, f(\lambda,\mathds{1}_b))_{1}\}$~~~$\rhd$~evaluate $f$ (train $\lambda$ for one step)
      
      \WHILE{$|H| < B$}
      
        \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}~~~$\rhd$~no model fitting in FT-PFN

        \STATE $\lambda' \xleftarrow{}$ \texttt{AF}($\hat{f},H,b_{\text{max}}$)~~~$\rhd$ {\color{red}\mfpirand} in \clftbo

        \STATE $y \leftarrow{} f(\lambda', b_{\lambda'}${\color{red}$+\mathds{1}_b$})~~~$\rhd$~evaluate $f$ (continue training $\lambda'$ for one more step)

        \STATE $H \leftarrow H \bigcup \{(\lambda', b_{\lambda'}+\mathds{1}_b, y)_{|H|+1}\}$

    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,b)\}_{(\lambda, b, f(\lambda,b)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}



==> icml2023/latex/algo_rebu_2col.tex <==
% \begin{algorithm}
%   \small
%   \caption{Freeze-thaw BO \label{algo:rebuttal-ftbo-copy}}
%   \textbf{Input:} 
%     configuration space $\Lambda$, \\
%     \textbf{Output:} $\lambda \in \Lambda$, obtaining the best performance \\
%   \textbf{Procedure:} HPO($\Lambda$, $f$, $\mathds{1}_b$, $b_{max}$, $B$): \\
%   \begin{algorithmic}
%       \STATE $\hat{f}\rightarrow{}$initialize surrogate modelp)
%       \WHILE{$|H| < B$}
%      \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}~~~$\rhd$~no model fitting in FT-PFN
%     \ENDWHILE \\
%     \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,b)\}_{(\lambda, b, f(\lambda,b)) \in H}$
%   %\ENDPROCEDURE
%   \end{algorithmic}
% \end{algorithm}



% \begin{algorithm}
% \small
%   \caption{\mfpirand{} \label{algo:rebuttal-mfpi-copy}}
%   \textbf{Input:} 
%     probabilistic surrogate $\hat{f}$, \\
%   \begin{algorithmic}
%       \STATE $f_{\text{best}} \leftarrow$ best score seen in $H$
%       \FORALL{$\hat{\lambda} \in \Lambda$}
%         \STATE $D \leftarrow{} D \bigcup{} \{(\hat{\lambda},~y')\}  $
%     \ENDFOR \\
%     \STATE \textbf{return} $\argmax_{\lambda \in \mathcal{X}} \{y\}_{(\lambda, y) \in D}$
%   %\ENDPROCEDURE
%   \end{algorithmic}
% \end{algorithm}




\begin{figure*}[htbp]
\centering
\begin{minipage}{0.48\textwidth}
  \begin{algorithm}[H]
 
\small
  \caption{Freeze-thaw BO \label{algo:rebuttal-ftbo}}
  \textbf{Input:} 
    configuration space $\Lambda$, \\
    measure of model performance $f$ to be minimized, \\
    value of unit step budget $\mathds{1}_b$,~~~$\rhd$~epoch(s)/update(s)\\
    maximal steps $b_{\text{max}}$,~~~$\rhd$~($\forall~\lambda \in \Lambda$)\\
    total HPO budget $B$ in training steps \\ 
    
    \textbf{Output:} $\lambda \in \Lambda$, obtaining the best performance \\
    
  \textbf{Procedure:} HPO($\Lambda$, $f$, $\mathds{1}_b$, $b_{max}$, $B$): \\
  \begin{algorithmic}
      \STATE $\hat{f}\rightarrow{}$initialize surrogate model
      \STATE $\lambda \sim \mathcal{U}(\Lambda) \hfill$~{\color{gray}initial random sample}
      \STATE $H \leftarrow{} \{(\lambda, \mathds{1}_b, f(\lambda,\mathds{1}_b))_{1}\}\hfill$~{\color{gray}evaluate $f$ (train $\lambda$ for one step)}
      
      \WHILE{$|H| < B$}
      
        \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}\hfill{\color{gray}no model fitting in FT-PFN}

        \STATE $\lambda' \xleftarrow{}$ \texttt{AF}($\Lambda,\hat{f},H,b_{\text{max}}$)\hfill {\color{gray}{\color{red}\mfpirand} in \clftbo}

        \STATE $y \leftarrow{} f(\lambda', b_{\lambda'}${\color{red}$+\mathds{1}_b$})\hfill{\color{gray}evaluate $f$ (thaw $\lambda'$ for $\mathds{1}_b$)}

        \STATE $H \leftarrow H \bigcup \{(\lambda', b_{\lambda'}+\mathds{1}_b, y)_{|H|+1}\}$

    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,b)\}_{(\lambda, b, f(\lambda,b)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
  \end{algorithm}
\end{minipage}\hfill
\begin{minipage}{0.48\textwidth}
  \begin{algorithm}[H]
  \small
  \caption{\mfpirand{} \label{algo:rebuttal-mfpi}}
  \textbf{Input:} 
    configuration space $\Lambda$, \\
    probabilistic surrogate $\hat{f}$, \\
    history of observations $H$, \\
    maximal steps $b_\text{max}$ \\
    
   \textbf{Output:} $\lambda' \in \Lambda$, next query \\
  
  \textbf{Procedure} \mfpirand($\hat{f}$, $H$): \\
  \begin{algorithmic}

      \STATE $f_{\text{best}} \leftarrow$ best score seen in $H$

      \STATE $z \sim \mathcal{U}(1, b_{\text{max}})$\hfill{\color{gray}random horizon}

      \STATE $\tau \sim \mathcal{U}(-4, -1)$\hfill{\color{gray}random threshold scaling}

      \STATE $f_{\text{threshold}} = f_{\text{best}} \cdot (1 - 10^\tau)$

      %\STATE $\mathcal{X} \rightarrow \{ \text{all unique}~\lambda~\text{in}~H \}$\hfill{\color{gray}generating candidate set}

      %\STATE $\mathcal{X} \leftarrow \mathcal{X} \bigcup{} \{\text{random samples from}~\Lambda\}$

      \STATE $D \leftarrow \{\}$ 
  
      % \STATE $\hat{f}\rightarrow{}$initialize surrogate model
      % \STATE $\lambda \sim \mathcal{U}(\Lambda)$
      % \STATE $H \leftarrow{} \{(\lambda, \mathd{1}_b, f(\lambda,\mathd{1}_b))_{1}\}$~~~$\rhd$~evaluate $f$
      \FORALL{$\hat{\lambda} \in \Lambda$}
      % \WHILE{$|H| < B$}

        \STATE $y' \leftarrow$ $\mathds{P}(\hat{f}(\hat{\lambda},~b_{\hat{\lambda}} + z) \le f_{\text{threshold}})$%~~~$\rhd$~\hfill{\color{gray}FT-PFN is trained for maximization and is handled accordingly in code
        % \mfpirand($\hat{\lambda}$, $b_{\hat{\lambda}} + z$, $f_{\text{threshold}}$)

        % \STATE $y' \leftarrow$ \mfpirand($\hat{\lambda}$, $b_{\hat{\lambda}} + z$, $f_{\text{threshold}}$)

        \STATE $D \leftarrow{} D \bigcup{} \{(\hat{\lambda},~y')\}  $
        % \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}~~~$\rhd$~no model fitting in FT-PFN

        % \STATE $\lambda' \xleftarrow{}$ \ {\color{red}\mfpirand}($\hat{f},H)$

        % \STATE $y \leftarrow{} f(\lambda', b_{\lambda'}${\color{red}$+\mathd{1}_b$})~~~$\rhd$~evaluate $f$

        % \STATE $H \leftarrow H \bigcup \{(\lambda', b_{\lambda'}+\mathd{1}_b, y)_{|H|+1}\}$

    \ENDFOR \\
    \STATE \textbf{return} $\argmax_{\lambda \in \Lambda} \{(\lambda, y)\}_{(\lambda, y) \in D}$
  %\ENDPROCEDURE
  \end{algorithmic}
  \end{algorithm}
\end{minipage}
% \captionsetup{labelformat=empty} % Remove "Figure X" label
% \caption*{Testing} % Custom caption
\end{figure*}

==> icml2023/latex/mf_pi_algo_rebu-copy.tex <==
\begin{algorithm}
\small
  \caption{\mfpirand{} \label{algo:rebuttal-mfpi-copy}}
  \textbf{Input:} 
    probabilistic surrogate $\hat{f}$, \\
  \begin{algorithmic}
      \STATE $f_{\text{best}} \leftarrow$ best score seen in $H$
      \FORALL{$\hat{\lambda} \in \Lambda$}
        \STATE $D \leftarrow{} D \bigcup{} \{(\hat{\lambda},~y')\}  $
    \ENDFOR \\
    \STATE \textbf{return} $\argmax_{\lambda \in \mathcal{X}} \{y\}_{(\lambda, y) \in D}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}



==> icml2023/latex/mf_pi_algo_rebu.tex <==
\begin{algorithm}

\small
  \caption{\mfpirand{} \label{algo:rebuttal-mfpi}}
  \textbf{Input:} 
    probabilistic surrogate $\hat{f}$, \\
    history of observations $H$, \\
    maximal steps $b_\text{max}$ \\
    
   \textbf{Output:} $\lambda' \in \Lambda$, next query \\
  
  \textbf{Procedure} \mfpirand($\hat{f}$, $H$):
  \begin{algorithmic}

      \STATE $f_{\text{best}} \leftarrow$ best score seen in $H$

      \STATE $z \sim \mathcal{U}(1, b_{\text{max}})$~~~$\rhd$~random horizon

      \STATE $\theta \sim \mathcal{U}(-4, -1)$~~~$\rhd$~random threshold scaling

      \STATE $f_{\text{threshold}} = f_{\text{best}} \cdot (1 - 10^\theta)$

      \STATE $\mathcal{X} \rightarrow \{ \text{all unique}~\lambda~\text{in}~H \}$~~~$\rhd$~generating candidate set

      \STATE $\mathcal{X} \leftarrow \mathcal{X} \bigcup{} \{\text{random samples from}~\Lambda\}$

      \STATE $D \leftarrow \{\}$ 
  
      % \STATE $\hat{f}\rightarrow{}$initialize surrogate model
      % \STATE $\lambda \sim \mathcal{U}(\Lambda)$
      % \STATE $H \leftarrow{} \{(\lambda, \mathd{1}_b, f(\lambda,\mathd{1}_b))_{1}\}$~~~$\rhd$~evaluate $f$
      \FORALL{$\hat{\lambda} \in \Lambda$}
      % \WHILE{$|H| < B$}

        \STATE $y' \leftarrow$ \mfpirand($\hat{\lambda}$, $b_{\hat{\lambda}} + z$, $f_{\text{threshold}}$)

        \STATE $D \leftarrow{} D \bigcup{} \{(\hat{\lambda},~y')\}  $
        % \STATE \setstcolor{red}\st{Train $\hat{f}$ on $H$}~~~$\rhd$~no model fitting in FT-PFN

        % \STATE $\lambda' \xleftarrow{}$ \ {\color{red}\mfpirand}($\hat{f},H)$

        % \STATE $y \leftarrow{} f(\lambda', b_{\lambda'}${\color{red}$+\mathd{1}_b$})~~~$\rhd$~evaluate $f$

        % \STATE $H \leftarrow H \bigcup \{(\lambda', b_{\lambda'}+\mathd{1}_b, y)_{|H|+1}\}$

    \ENDFOR \\
    \STATE \textbf{return} $\argmax_{\lambda \in \mathcal{X}} \{y\}_{(\lambda, y) \in D}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}



==> icml2023/latex/mfpi_method_rebu.tex <==

% \editmode{
% Let \texttt{AF} be a general acquisition function, $\lambda \in \Lambda$ be a hyperparameter, $z \in \mathcal{Z}$ a fidelity such as the number of training steps, $f_{\text{best}}$ is the best seen performance, $b_{\text{max}}$ is the maximum training steps available to a $\lambda$, and $f$ is the surrogate model trained on the observations $H$.
% }
% % Let \texttt{AF} represent a general acquisition function, $\lambda \in \Lambda$ be a hyperparameter, $z \in \mathcal{Z}$ be a fidelity, $f_{\text{threshold}}$ be the best seen performance till current iteration, and $f$ be the surrogate model trained on the observations collected.
% \editmode{
% \begin{equation} \label{eq:rebut-eq-af}
%     \texttt{AF}(\lambda, f_{\text{threshold}}): \Lambda \rightarrow \mathbb{R}\text{,}
% \end{equation}
% }
% \editmode{
% is a general acquisition function, with $f_{\text{threshold}} \sim{}$ a function of $f_{\text{best}}$. Now, a general multi-fidelity acquisition function can be denoted as,
% }
% \editmode{
% \begin{equation} \label{eq:rebut-eq-mf-af}
%     \texttt{MF-AF}(\lambda, z, f_{\text{threshold}}): \Lambda \times ~\mathcal{Z} \rightarrow \mathbb{R}\text{.}
% \end{equation}
% }
% \editmode{
% When $z=b_{\text{max}}$ and $f_{\text{threshold}}=f_{\text{best}}$, any vanilla AF such as Expected Improvement (EI) or Probability of Improvement (PI)~\citep{mockus-tgo78a} is recovered from Equation~\ref{eq:rebut-eq-mf-af}.
% To adapt to the freeze-thaw scenario and allow every configuration explored to have a chance for re-selection (thawing) we randomize the extrapolation length ($z$) and the difficulty of the improvement threshold ($f_{\text{threshold}}$), and apply PI for,
% }
% \editmode{
% \begin{equation} \label{eq:rebut-eq-mf-af-random}
%     \texttt{MFPI-random}(\lambda, z^{\text{rand}}, f_{\text{threshold}}^{\text{rand}}): \Lambda \times ~\mathcal{Z} \rightarrow \mathbb{R}\text{,}
% \end{equation}
% }
% \editmode{
% where $z^{\text{rand}} \sim \mathcal{U}(1, b_{\text{max}})$ is the sampled extrapolation horizon, and $f_{\text{threshold}}^{\text{rand}} = f_{\texttt{best}} \cdot (1 - \tau)$, with $log_{10}(\tau) \sim \mathcal{U}(-4, -1)$ as the sampled scaling for the threshold. 
% }

% \editmode{
% In Section~\ref{sec:ablate_acquisition} we empirically compare the different choices for parameterizing Equation~\ref{eq:rebut-eq-mf-af} compared to our choice in Equation~\ref{eq:rebut-eq-mf-af-random}.
% In Appendix~\ref{app:af} we give the pseudo-code and present further ablations in Appendix~\ref{app:ablations}.
% }

%%%%%%%%%%%%%%%
\editmode{Following the Freeze-Thaw Bayesian Optimization framework (Section~\ref{sec:ftbo}), we continue training the configuration $\lambda\in\Lambda$ that maximizes some acquisition function.
%Here, we assume a general multi-fidelity (MF) acquisition function (AF) represented as,
}
\editmode{
\begin{equation} \label{eq:rebut-eq-mf-af}
    \texttt{MF-AF}(\lambda, z~|~f_{\text{threshold}}): \Lambda \times ~\mathcal{Z} \rightarrow \mathbb{R}\text{,}
\end{equation}
}
\editmode{
where \texttt{AF} is a general acquisition function, 
$\lambda \in \Lambda$ a hyperparameter configuration, 
$z \in \mathcal{Z}$ the fidelity (e.g. number of training steps), 
and $f_{\text{threshold}}$ a function of $f_{\text{best}}$ (best observed performance).
% $f_{\text{best}}$ $\leftarrow$ best seen performance, 
% $b_{\text{max}}$ $\leftarrow$ maximum training steps available to a $\lambda$, 
% and $f$ $\leftarrow$ surrogate model trained on the observations $H$.
For example, fixing $z=b_{\text{max}}$ and $f_{\text{threshold}}=f_{\text{best}}$, recovers a vanilla AF such as Expected Improvement (EI) or Probability of Improvement (PI)~\citep{mockus-tgo78a}.
}

% The quality of uncertainty calibration of surrogate predictions depend on the task at hand, quality of the surrogate training set, and the extrapolation length (horizon), while the AF score is calibrated by the dynamic improvement threshold.
% Instead of a fixed setting for these choices (horizon, threshold) we randomize these choices from a predefined range.
% While integrating/marginalizing across different thresholds of improvement would result in EI, sampling allows a greater amount of diversification.
% Hedging these choice from a portfolio of AFs in each iteration is helpful under the freeze-thaw setup where actual queries made are more granular (L7 in Alg.~\ref{algo:ftbo}) than standard BO.
% Thus, we have a relatively simple, parameter-free AF with a good exploration-exploitation balance in,
\editmode{
The quality of uncertainty calibration in surrogate predictions depends on the task, surrogate training set quality, and extrapolation length (horizon). 
Meanwhile, the AF score is calibrated by an improvement threshold. 
In our work, we choose PI as the base AF as it is less likely to drive search towards high uncertainty regions along the hyperparameter and fidelity subspaces.
Instead of using a fixed threshold or a fixed extrapolation horizon for this PI calculation, we explore a range of possible thresholds and horizons by random sampling from either fixed or problem-specific bounds.
Such sampling procedure is undertaken every iteration and is akin to an acquisition selection from a portfolio of different PIs.
In contrast to integrating over all thresholds (leading to Expected Improvement, EI), this allows for greater diversification in the exploration process.
}
\editmode{
We posit that this hedging with a portfolio of AFs in each iteration benefits freeze-thaw setups where queries are more granular than standard BO. 
The result is a simple, parameter-free AF with a balanced exploration-exploitation trade-off,
}
% Two critical choices determining behaviour of the exact acquisition are: (i) \textit{extrapolation horizon} that determines prediction uncertainty (more uncertainty with longer horizons); (ii) \textit{improvement threshold} that calibrates improvement over best-seen scores, favoring larger improvements.

% The best setting of these two choices critically depends on the task at hand and the stage of the optimization. 
% In order to hedge, and use a portfolio of acquisition functions in each iteration, we draw both of these choices uniformly at random from a predefined range. 
% While integrating/marginalizing across different thresholds of improvement would result in EI, sampling allows a greater amount of diversification.
% This hedging is very helpful since in the freeze-thaw setup our individual decisions are much more granular than in standard Bayesian optimization (BO), and the simple sampling of both of these choices results in a relatively simple, parameter-free acquisition with a good exploration-exploitation balance in,
\editmode{
\begin{equation} \label{eq:rebut-eq-mf-af-random}
    \texttt{MFPI-random}(\lambda, z^{\text{rand}}~|~f_{\text{threshold}}^{\text{rand}}): \Lambda \times ~\mathcal{Z}\rightarrow \mathbb{R}\text{,}
\end{equation}
}
\editmode{
which evaluates to the predicted likelihood that a candidate configuration $\lambda \in \Lambda$ after $z^{\text{rand}}$ \textit{more} steps of training obtains a model exceeding the $f_{\text{threshold}}^{\text{rand}}$ performance threshold, 
where $z^{\text{rand}} \sim \mathcal{U}(1, b_{\text{max}})$ is the sampled extrapolation horizon, and $f_{\text{threshold}}^{\text{rand}} = f_{\text{best}} \cdot (1 - \tau)$, with $log_{10}(\tau) \sim \mathcal{U}(-4, -1)$ as the sampled scaling for the threshold. Further details, as well as pseudo code (Algorithm~\ref{algo:mf-af}) can be found in Appendix~\ref{app:af}.
}

==> icml2023/latex/table_quality_surrogates.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.88\textwidth}{!}{\begin{tabular}{
  l
  l
  S[table-format=-2.3]
  S[table-format=1.3]
  S[table-format=-2.3]
  S[table-format=1.3]
  S[table-format=3.3, table-comparator=true]
  S[table-format=1.3]
  S[table-format=2.3]
}
\toprule
& & \multicolumn{2}{c}{LCBench} & \multicolumn{2}{c}{PD1} & \multicolumn{2}{c}{Taskset} & \multicolumn{1}{c}{\textbf{Runtime (s)}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} %\cmidrule(lr){9-9}
\textbf{\# samples} & \textbf{Method} & {\textbf{Log-likelihood}} & {\textbf{MSE}} & {\textbf{Log-likelihood}} & {\textbf{MSE}} & {\textbf{Log-likelihood}} & {\textbf{MSE}} & {\textbf{}} \\
\midrule
\multirow{4}{*}{100} & DPL & -10.401 & 0.007 & -30.286 & 0.047 & -15.496 & 0.003 & 4.525 \\
 & DyHPO & -0.377 & 0.020 & -0.411 & 0.071 & -0.371 & 0.004 & 4.964 \\
 & FT-PFN (no HPs) & 1.334 & 0.011 & 0.880 & 0.054 & 3.156 & 0.003 & 0.262 \\
 & FT-PFN & 1.582 & 0.006 & 0.872 & 0.039 & 3.272 & 0.003 & 0.264 \\
\midrule
\multirow{4}{*}{200} & DPL & -7.502 & 0.005 & -22.207 & 0.039 & -13.870 & 0.003 & 8.742 \\
 & DyHPO & -0.359 & 0.013 & -0.399 & 0.062 & -0.355 & 0.004 & 7.064 \\
 & FT-PFN (no HPs) & 1.547 & 0.009 & 1.100 & 0.040 & 3.306 & 0.002 & 0.285 \\
 & FT-PFN & 1.906 & 0.004 & 1.064 & 0.029 & 3.447 & 0.002 & 0.285 \\
\midrule
\multirow{4}{*}{400} & DPL & -8.056 & 0.004 & -17.956 & 0.027 & -11.874 & 0.002 & 15.605 \\
 & DyHPO & -0.347 & 0.009 & -0.389 & 0.050 & -0.344 & 0.003 & 15.125 \\
 & FT-PFN (no HPs) & 1.791 & 0.007 & 1.485 & 0.028 & 3.481 & 0.002 & 0.330 \\
 & FT-PFN & 2.198 & 0.003 & 1.401 & 0.020 & 3.582 & 0.002 & 0.344 \\
\midrule
\multirow[c]{4}{*}{800} & DPL & -6.699 & 0.003 & -11.101 & 0.018 & -7.835 & 0.001 & 29.256 \\
 & DyHPO & -0.337 & 0.006 & -0.374 & 0.030 & -0.336 & 0.003 & 54.354 \\
 & FT-PFN (no HPs) & 2.105 & 0.005 & 2.146 & 0.012 & 3.713 & 0.001 & 0.453 \\
 & FT-PFN & 2.523 & 0.002 & 1.879 & 0.011 & 3.696 & 0.001 & 0.474 \\
\bottomrule
\end{tabular}}
\caption{Comparison of \ftpfn, a variant of \ftpfn\ that excludes hyperparameters, \dyhpo\ and \dpl\ accross three benchamrks. Performance metrics include log-likelihood and mean squared error (MSE) as well as the runtime of predictions. Values represent the median over tasks.}
\label{tab:quality_predictions}
\end{table*}

==> icml2023/old_sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we proposed \ftpfn{} a novel surrogate for freeze-thaw Bayesian optimization. We showed that the point and uncertainty estimates produced by \ftpfn{} through \emph{in-context learning} are superior to those obtained by fitting/training recently proposed deep Gaussian process~\citep{wistuba-neurips22} and deep power law ensemble~\citep{kadra-neurips23} models, while being over an order of magnitude faster. We presented the first-ever empirical comparison of different freeze-thaw implementations. Our results confirm the superiority of these HPO methods, in the low-budget regime, and show that our in-context learning approach is competitive with the state-of-the-art.

Despite our promising results,
% MORE DATA
we admit that attaining the sample efficiency required to scale up to modern deep learning (e.g., LMM pretraining) remains a challenging endeavor. Future work should attempt to extend our approach to take advantage of additional sources of prior information, e.g., 
%meta-learning
to do in-context meta-learning, leveraging learning curves on related tasks~\citep{ruhkopf-tmlr22}; 
%user priors
to incorporate user priors~\citep{muller-icml23a,mallik2023priorband};
%white-box
and additional information about the training process (e.g., gradient statistics).
% PARALLEL
An alternative to scaling up is scaling in parallel. Here, we expect our in-context learning approach to reduce the overhead further, as the online learning/refitting stage occurs on the critical path, while in-context learning during prediction can easily be parallelized.
% The current 
Finally, the current \ftpfn{} model has some limitations. First, due to context size constraints, it is only trained for HPO budgets of up to 1,000 steps; it requires the performance metric and each hyperparameter value to be normalized in [0,1]; and supports up to 10 hyperparameters. While we believe that this is reasonable, future work building systems should push these limits, train larger models, on more data, and explore ways to scale to larger context sizes.
% TODO: Acquisition function
% TODO: Add something about scaling laws?
% Closing statement
In summary, there is a lot left unexplored, and we hope that the relative simplicity, efficiency, and public availability of our method, lowers the threshold for future research in this direction.

\iffalse
\paragraph{Future work/limitations:}
\begin{itemize}
    \item Non-myopic / parallel acquisition (PFNs4BO)
    \item Meta-learning / Context size limit (MASIF)
    \item Beyond training time / Scaling laws (DPL, tuning as we scale)
    \item Beyond learning curves
    \item Cost-awareness
    \item Categorical, conditional hyperparameters (normalization etc
    \item Learning the acquisition
    \item designing priors
    \item User priors (Priorband, $\pi$BO)
\end{itemize}
\fi

==> icml2023/old_sections/experiments.tex <==

\input{icml2023/latex/table_quality_surrogates}

\section{Experiments}
\label{sec:exp}

In this section, we compare \ours\ to state-of-the-art multi-fidelity 
%and publicly available 
freeze-thaw Bayesian optimization methods.
%implementations. 
To this end, we first assess \ftpfn\ in terms of the quality and cost of its prediction (Section~\ref{sec:quality_surrogate}). Then, we assess our approach, which combines \ftpfn\ with our \mfpirand\ acquisition function, on HPO tasks (Section~\ref{sec:sota}). Finally, we conduct an ablation study on acquisition function used in \ours\ (Section~\ref{sec:ablate_acquisition}).

Our main baselines are both other recent freeze-thaw approaches: \dyhpo\ \cite{wistuba-neurips22} and \dpl\ \cite{kadra-neurips23}. We use the publicly available implementations for \dyhpo\ and \dpl\
with default hyperparameter values.
%For diversity, we also include popular multi-fidelity  (Hyperband ASHA, and GP-based BO) and Black-box (uniform random search) methods. %A comprehensive description of the baselines is presented in Appendix~\ref{a:baselines}.

We conduct our experiments on three benchmarks: \lcbench\ \cite{zimmer-ieee2021a}, \pdone{}~\cite{wang-arxiv21a}, and \taskset~\cite{metz-arxiv20b}. These benchmarks, covering different architectures (Transformers, CNNs, MLPs) and tasks (NLP, vision, tabular data), are commonly used in the HPO literature and are also used by our baselines. A detailed overview of the tasks included in each benchmark is presented in Appendix~\ref{a:benchmarks}.



\subsection{Cost and Quality of Predictions}
\label{sec:quality_surrogate}

In this section, we compare the predictive capabilities of \ftpfn\ to that of existing surrogate models, including the deep Gaussian process of \dyhpo{}~\cite{wistuba-neurips22} and the deep ensemble of power laws model of \dpl{}~\cite{kadra-neurips23}. We also consider a variant of \ftpfn\ trained on the same prior, but not taking the hyperparameters as input (referred to as "no HPs"). This variant bases its predictions solely on a set of partially observed learning curves.

\paragraph{Evaluation procedure:} From a given benchmark, we sample both a set of partial curves, where each curve has its own set of target epochs. The selection process is strategically designed to encompass a wide range of scenarios, varying from depth-first approaches, which involve a smaller number of long curves, to breadth-first approaches, where multiple shorter curves are explored. Additional details on the sampling strategy can be found in Appendix~\ref{a:priorgen}. 
Once we have compiled the partial curves and their corresponding hyperparameter values, we will input them into \ftpfn\ as context samples and training data for DyHPO and DPL. We will then request each of the surrogate models to predict performance at the target epochs. To assess the quality of the predictions, we will utilize two metrics: log-likelihood (log-score, the higher the better), measuring the approximation of the posterior distribution ($\sim$ uncertainty calibration), and mean squared error (the lower the better), measuring the accuracy of point predictions. Additionally, we also report the runtime, accounting for fitting and predicting parts, of each surrogate. The evaluation was run on a single \texttt{Intel Xeon 6242 CPU}.

\paragraph{Results discussion:} Table~\ref{tab:quality_predictions} presents the log-likelihood and MSE (Mean Squared Error) for each approach relative to the context sample size. As expected, we observe an increase in log-likelihood and a decrease in MSE as the context size get larger. Notably, \ftpfn\ and its No HPs variant significantly outperform \dpl\ and \dyhpo\ in terms of log-likelihood. \dpl\ in particular has very low log-likelihood values, corresponding to a poor uncertainty estimate such as being overly confident in incorrect predictions. This may due to the very low of ensemble size ($=5$) adopted by \cite{kadra-neurips23} compounded by the strong power law assumption of the approach. On the other hand, \dyhpo\ struggles with low log-likelihood due to its inability to extrapolate beyond a single step effectively. Intriguingly, for larger context sizes on \pdone{} and \taskset{}, the No HPs variant of \ftpfn\ achieves superior log-likelihood compared to \ftpfn\ itself, suggesting that in these cases, direct observations are more informative than hyperparameter values. 
Regarding MSE, \ftpfn\ generally surpasses the baselines in \lcbench{} and \pdone{}, performing comparably to \dpl\ on \taskset{}. Meanwhile, \dyhpo\ is outperformed by the No HPs version of \ftpfn.

\begin{figure*}
  \includegraphics[width=0.9\textwidth]{icml2023/figures/all_combined.png}\centering
  \caption{Comparison of our method against state-of-the-art baselines on all 3 benchmarks. First row shows normalized regret aggregated across multiple tasks in each benchmark (See Appendix \ref{a:benchmarks} for benchmark details, and the results per task can be found in Appendix~\ref{a:per_task_plot}). Second row shows the average ranks of each method. \label{fig:per-bench-sota}}
\end{figure*}

Beyond the impressive log-likelihood and MSE results, our approach also yield significant speed advantages over the baseline methods. Depending on the context sample size, our method achieves speedups ranging from $10\times$ to $100\times$ faster than both \dpl\ and \dyhpo.  

\subsection{Assessment of HPO performance}
\label{sec:sota}

In this section, we present an extensive empirical comparison, showing the merits of our method on HPO tasks across a variety of \textbf{tabular} benchmarks (see Appendix~\ref{a:benchmarks}) in the low budget regime. Additionally to \dpl\ and \dyhpo, we include Hyperband, ASHA, Gaussian Process-based FT-BO (using \dyhpo's one-step EI acquisition function) and uniform random search, as baselines. Each algorithm is allocated a total budget of 1000 steps for every task, which corresponds to 20 full trainings on \lcbench\ and \taskset\, with each task being repeated 10 times, each time starting from a different random configuration (see Algorithm~\ref{algo:ftbo}). We report two complementary metrics: The normalized regret, capturing performance differences, and the average rank of each method, capturing the relative order. Formally, the normalized regret corresponds to a $[0, 1]$ normalization of the observed error w.r.t to the best (lowest) and worst (highest) errors recorded by all algorithms on the task. % This metric not only reflects task difficulty but also encourages competition among the methods. For the average ranks, methods are ranked for each run (seed) and then averaged across both seeds and tasks.  


\paragraph{Results discussion:}  Figure~\ref{fig:per-bench-sota} presents the comparative results per benchmark.  The results validate the superiority of freeze-thaw approaches (\ours, \dyhpo, and \dpl) compared to standard approaches (Hyperband, ASHA, and uniform random search) for low-budget settings. Most notably, these results establish the promise of \ours, which either outperforms (on \lcbench{} and \taskset{}) or competes closely (on \pdone{}) with \dpl{} and \dyhpo{}. \ours\ is also consistently the best on average rank after $400$ optimization steps across the benchmarks. 
For an in-depth presentation, Appendix~\ref{a:per_task_plot} (Figures~\ref{fig:per-task-lcb1}-\ref{fig:per-task-taskset2}) offers a closer look at the raw error metrics for each algorithm across individual tasks. These detailed results collectively confirm the robustness of \ours\ for HPO tasks, showing its ability to compete if not outperform the most competitive baselines.

%Check Figures \ref{fig:aggregate-sota} and \ref{fig:per-bench-sota}.
\iffalse
\subsection{Ablation on surrogate (?)}
\label{sec:ablate_surrogate}
Here, we would evaluate our method combined with different surrogates(see Appendix~\ref{a:surrogate}) across a variety of \textbf{tabular} benchmarks (see Appendix~\ref{a:tabular}) to get some insight into their relative contribution. A full grid evaluation (ablating on surrogates/acquisition policy resp.) in Appendix.
\fi 
\subsection{Ablation on Acquisition}
\label{sec:ablate_acquisition}

\input{icml2023/figures/af_ablation}

In this section, we evaluate how \ours{} performs in combination with other acquisition functions and aim to assess to what extent our novel acquisition function described in Section~\ref{sec:acquisition} contributes to its HPO success. To this end, we consider \ours{} variants combining \ftpfn{} with 
and comparing performance against the EI-based acquisitions used in prior-art~\citep{wistuba-neurips22,kadra-neurips23}, i.e., \mfei{} predicting one step in the future (\dyhpo{}), and \eimax{} predicting at the highest budget $b_{max}$ (\dpl{}). We also include their PI counterparts \mfpi{} and \pimax{}, as well as variants of \mfpirand{} that only vary the prediction horizon, \pirandh{} with $T=0$, or only vary the threshold, \pirandt{} with $h = b_{max}$. Apart from the methods compared, the experimental setup is identical to that in Section~\ref{sec:sota}.

\paragraph{Results discussion:} Figure~\ref{fig:af_ablate} shows the comprehensive results for our $\clftbo{}$ variants for each of the benchmarks, in terms of average ranks and average normalized regrets, aggregated across all tasks. Generally, we find that performance varies strongly between acquisitions, suggesting this choice is at least as important for HPO success as our surrogate's superior predictive quality. In particular, we find that combinations with the EI-based acquisitions \mfei{} and \eimax{} proposed in prior-art, are amongst the worst-performing variants, both in terms of rank and regret. For example, \eimax{} fails on \lcbench{} and \pdone{}, while \mfei{} fails on \pdone{} and \taskset{}. Curiously, these trends do not seem to extend to our baselines, e.g., \dpl{} using \eimax{} performs strongly on \lcbench{} and \dyhpo{} using \mfei{} performs strongly on \pdone{}. We conjecture that this failure is related to the (justified) lack of confidence $\ftpfn{}$ has about its predictions, as is evident by the superior log-scores in Table~\ref{tab:quality_predictions}. As a result, the predicted posterior will be heavy-tailed, resulting in the high EI values for those configurations our predictions are least confident for. While this drives exploration, in the very low budget regime, it can easily lead to a catastrophic failure to exploit.

Overall, we find that while some variants are successful at specific tasks, in very early stages of the optimization, none exhibit the same robustness in performance across benchmarks, making \mfpirand{} the clear winner in this comparison.


\iffalse
%DyHPO / DPL
%variants thereof using PI instead of EI ().
%variants of Pi-random, randomizing only the horizon (T=0), and PI-random randomizing only the threhsold, fixing horizon to max.
Here, we would evaluate our method combined with different acquisition function (see Appendix~\ref{a:acquisition}) across a variety of \textbf{tabular} benchmarks (see Appendix~\ref{a:tabular}) to get some insight into their relative contribution. A full grid evaluation (ablating on surrogates/acquisition policy resp.) in Appendix.

\subsection{Evaluation in continuous settings}
Here, we evaluate specific combinations (acquisition+surrogate) on continuous/mixed state spaces from Appendix~\ref{a:surrogate}, combining them with different optimizers that support such spaces. Again, the full grid in Appendix.


\subsection{Quantify Overhead}
We would quantify cost of 
\fi

==> icml2023/old_sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Hyperparameters are essential in deep learning to achieve strong model performance. However, due to the increasing complexity of these models, it is becoming more challenging to find promising hyperparameter settings, even with the help of hyperparameter optimization (HPO, Section~\ref{sec:hpo}) tools~\citep{feurer-automlbook19a,bischl-hpo23}. Traditional HPO techniques using Bayesian optimization are unsuitable for modern deep learning because they treat the problem as a black box, making it computationally expensive since they require a full model training for each evaluation. 

Recent research in HPO has shifted towards multi-fidelity methods~\cite{li-iclr17a,li-arxiv20a,falkner-icml18a,klein-arxiv20a,li-mlsys20a,awad-ijcai21a}, utilizing lower fidelity proxies (e.g., training for fewer steps, using less data, smaller models) and only evaluating the most promising hyperparameter settings at the full fidelity. While these methods have potential, they often use coarse-grained fidelity spaces and rely on the rank correlation of performances across fidelities. Moreover, they do not fully utilize the anytime nature of algorithms such as checkpointing, continuation, and extrapolation. As a result, these methods struggle to allocate computational resources efficiently, leading to suboptimal performance in many scenarios.

The freeze-thaw Bayesian optimization method (\ftbo{}, Section~\ref{sec:ftbo}), originally proposed by ~\citet{swersky-arxiv14a}, is a promising approach to efficiently allocate computational resources by pausing and resuming the evaluation of different hyperparameter configurations. This method is an improvement over traditional grey-box methods as it dynamically manages resources, and recent implementations~\citep{wistuba-neurips22,kadra-neurips23} hold the state-of-the-art in the low-budget regime ($\sim$ 20 full function evaluations). However, these contemporary implementations (\olftbo{}) have limitations. In particular, they rely on online learning to update the surrogate model at each step which can lead high computational overhead, instability, and complexity in managing additional hyper-hyperparameters. Moreover, they also suffer from strong assumptions about learning curves, which may not be applicable in all scenarios, resulting in overly confident incorrect predictions.

\input{icml2023/figures/ftpfn_example}

In this work, we leverage prior-data fitted networks \citep[PFNs]{muller-iclr22a} (Section~\ref{sec:pfn}), a Transformer-based meta-learning approach to Bayesian inference, to enhance freeze-thaw Bayesian optimization through in-context learning. Our PFN model (\ftpfn{}) infers the task-specific relationship between hyperparameter settings and their learning curves in a single forward pass, eliminating the need for online training during the search. This approach directly addresses key challenges in traditional HPO methods, lowering computational overhead and stabilizing the optimization process. The contributions of this paper are as follows.

\begin{itemize}
\item We propose \ftpfn{} (Section~\ref{sec:surrogate}), a new surrogate model for freeze-thaw Bayesian optimization, replacing online learning with in-context learning using PFNs.
\item We train a single model \ftpfn{} using only synthetic data, generated to mimic realistic HPO learning curves, that we use in all of our experiments covering a wide variety of HPO tasks. We open-source the trained model alongside the code used for training it: \url{https://anonymous.4open.science/r/CL-FT-BO-C606}
\item We empirically show that this \ftpfn{} outperforms existing surrogates, at point prediction and posterior distribution approximation, while being over an order of magnitude faster, and despite never having been trained on real HPO data (Section~\ref{sec:quality_surrogate}). A qualitative example of the predictions made by our model is shown in Figure~\ref{fig:example}.
\item We combine \ftpfn{} with a novel acquisition function (\mfpirand{}, Section~\ref{sec:acquisition}) and find that the resulting in-context freeze-thaw method (\clftbo{}) 
yields a new state-of-the-art performance 
%is as good or better than the previous best HPO method, 
on 
%each of 
the three benchmark suites for HPO for deep learning (\lcbench{}, \taskset{}, \pdone{}) considered by \citet{kadra-neurips23}, in the same low-budget regime.
%\item We perform extensive ablation experiments to evaluate various combinations of freeze-thaw surrogates and acquisition strategies. These experiments provide valuable insights into their relative performance and the interaction effects, contributing to a deeper understanding of the HPO process.
\end{itemize}


\begin{comment}
\begin{itemize}
    \item Hyperparameters matter in deep learning. 
    \item Automated HPO does not scale up to modern DL:
    \begin{itemize}
    \item Cost of evaluation
    \item HPO mostly black-box optimization
    \end{itemize}
    \item Grey-box/multi-fidelity HPO and shortcomings.
    %\item Better Utilize the specific properties of the DL domain (continuations, freeze-thaw, learning curves), incorporating the inductive biases from the literature (priors).
    \item Exception: Freeze-Thaw Bayesian Optimization
    \begin{itemize}
    \item Explain the concept
    \item Recently: DyHPO and DPL
    \item Shortcomings Sota: 
    \begin{itemize}
    \item Focus: Online learning (overhead, stability, hyper-hyperparameters)
    \item Side: Strong assumptions on learning curves 
    \item Side: No support for continuous spaces
    \end{itemize}
    \end{itemize}
    \item In this work: In-context learning using PFNs.
\begin{itemize}
\item Explain concepts
\item How this addresses the aforementioned issues
\end{itemize}
\item Our contributions:
\begin{itemize}
\item We propose HPO-LC-PFN a new surrogate model for Freeze-Thaw Bayesian Optimization, replacing online with in-context learning using PFNs.
\item We propose a novel acquisition policy for Freeze-Thaw Bayesian Optimization, supporting continuous search spaces and leveraging HPO-LC-PFN's superior extrapolation capabilities to choose appropriately when to sample or promote.  
\item We show that the resulting method (surrogate + acquisition) outperforms all existing HPO methods in the low-budget regime ($<$ 20 full evaluations).
\item We perform extensive ablation experiments, evaluating other combinations of dynamic surrogates and acquisitions, providing valuable insights into their relative performance and interaction effects.
\item We use this method to tune a model (babyGPT or HPO-LC-PFN), improving its performance...
\item We open-source our code
\end{itemize}
\end{itemize}
\end{comment}

==> icml2023/old_sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

We now discuss some preliminaries that we build on more formally, introducing our notation on the way.
\subsection{Hyperparameter Optimization (HPO)}
\label{sec:hpo}
Consider an iterative machine training pipeline with configurable hyperparameters $\lambda \in \Lambda$. E.g., when training a neural network using gradient descent we could configure the learning rate, weight decay, dropout rate, etc.
Let $f(\lambda,t)$ be some measure of downstream performance (e.g., validation loss) of the model obtained after $t$ steps of training (e.g., epochs), using hyperparameter settings $\lambda$, that we would like to minimize. Further, assume that each training run is limited to $b_{max}$ such training steps. HPO aims to find a hyperparameter setting producing the best model, i.e., $
\lambda^* = \argmin_{\lambda \in \Lambda} \min_{0 \leq t \leq b_{max}} f(\lambda, t)$, within the limited total optimization budget of $B$ training steps. Note that in modern deep learning, we typically have $B \ll |\Lambda| \cdot b_{max}$; the budget available for HPO often does  not allow us to execute more than a few full training runs. In this setting, the crux of HPO lies in allocating these limited training resources to the most promising hyperparameter settings, i.e., to find an allocation $\{b_\lambda\}_{\lambda \in \Lambda,\, 0 \leq b_{\lambda} \leq b_{max}}$ with $\sum_{\lambda \in \Lambda} b_{\lambda'} = B$ that minimizes $\min_{\lambda \in \Lambda,\, 0 \leq t \leq b_{\lambda}} f(\lambda, t)$.

\subsection{Freeze-Thaw Bayesian Optimization (\ftbo{})}
\label{sec:ftbo}
As discussed above, 
\citet{swersky-arxiv14a} proposed to address this challenge by following a fine-grained dynamic scheduling approach, allocating resources to configurations ``one step at a time''. More specifically, at each step it uses its history $H = \{\lambda, t, f(\lambda, t)\}_{t=1, \forall \lambda \in \Lambda}^{b_\lambda'}$, the various partial learning curves observed thus far in the current partial allocation $\{b_\lambda'\}_{\lambda \in \Lambda}$, to fit a dynamic Bayesian surrogate model $g(\lambda, t) \approx \Pr(f(\lambda, t) \,|\, H)$ for $t > b_\lambda'$ that probabilistically extrapolates the partially seen performance of configuration $\lambda$ beyond $b_\lambda'$.
%, i.e., a probabilistic model predicting the distribution of model performances obtained when allocating further resources to the training using $\lambda$. 
Following the BO framework, it decides which of these to continue (or start if $b_{\lambda} = 0$) as $\argmax_{\lambda \in \Lambda} a(\{(\lambda, t, g(\lambda,t)\}_{t > b_\lambda})$, where $a$ is a dynamic acquisition function trading off exploration and exploitation. Algorithm~\ref{algo:ftbo} shows the freeze-thaw Bayesian optimization framework (\ftbo{}), contrasted with a traditional black box Bayesian Optimization (\bbbo{}) loop. Here, the crucial difference lies in that resources in \ftbo{} are allocated one training step, rather than one full training, at the time. Note that \ftbo{} assumes training to be preemptive, i.e., that we can stop (\emph{freeze}) a model training, and continue (\emph{thaw}) it later; this assumption is reasonable in modern deep learning where checkpointing is common practice.
\iffalse
\paragraph{Assumptions:}
We assume an iterative preemptive training, where each iteration is roughly equally expensive and the model measure performance can be observed after every iteration.
We assume a finite set of hyperparameter settings $\Theta$
We assume training 
We assume $\lambda$ to be numeric. These setting is commonplace in Similar assumptions were made in recent prior art and relaxing these was out of scope.
\fi

\begin{comment}
    

\begin{algorithm}
\small
  \caption{Freeze-thaw vs. Black box BO \label{algo:ftbo}}
  Contrasts the online learning (\textcolor{green}{\olftbo}), our in-context learning Freeze-thaw (\textcolor{blue}{\ours}), and black box (\textcolor{red}{\bbbo{}}) approaches to Bayesian optimization for HPO. Code specific to these methods is shown in \textcolor{green}{green}, \textcolor{blue}{blue}, and \textcolor{red}{red}, respectively. Code shared by all methods is shown in black, code shared between both \textcolor{teal}{\ftbo{}} variants in \textcolor{teal}{blue green}, and code shared between \bbbo{} and \olftbo{} (\textcolor{brown}{not \ours}) in \textcolor{brown}{brown} \\
  \textbf{Input:} The configuration space $\Lambda$ \\
  \textbf{Input:} The measure of model performance $f$ to be minimized \\
  \textbf{Input:} The maximal training run length $b_{max}$ in training steps \\
  \textbf{Input:} The total HPO budget $B$ in training steps \\
  \textbf{Component:} The \textcolor{teal}{dynamic} surrogate model $g$ \\
  \textbf{Component:} The \textcolor{teal}{dynamic} acquisition function $a$ \\
  \textbf{Output:} The configuration $\lambda \in \Lambda$ obtaining the best model \\
  \textbf{Procedure} HPO($\Lambda$, $f$, $b_{max}$, $B$):
  \begin{algorithmic}
      \STATE $\lambda \sim \mathcal{U}(\Lambda)$
      \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
      \STATE \textcolor{teal}{$H = \{(\lambda, 1, f(\lambda,1))\} \gets {\sc evaluateFT}(\lambda)$}
      \WHILE{$|H| < B$}
        \STATE \textcolor{brown}{g.fit(H)} \textcolor{blue}{\COMMENT{\ours{} does not require refitting the PFN}}
        \STATE $\Lambda' = \{\lambda\}_{\lambda \in \Lambda:\, (\lambda, b_{max}, \cdot) \notin H}$
        \STATE \textcolor{red}{$P = \{\lambda,\,g(\lambda)\}_{\lambda \in \Lambda'}$}
        \STATE \textcolor{teal}{$P = \{\lambda,t,\,g(\lambda,t\textcolor{blue}{,H})\}_{\lambda \in \Lambda',\, t > b_\lambda}$}
        \STATE $\lambda = \argmax_{\lambda \in \Lambda'} a(P)$
        \STATE \textcolor{red}{$H = \{\lambda, t, f(\lambda,t)\}_{t=1}^{b_{max}} \gets {\sc evaluateBB}(\lambda)$}
        \STATE \textcolor{teal}{$H = \{(\lambda, b_\lambda+1, f(\lambda,b_\lambda+1))\} \gets {\sc evaluateFT}(\lambda)$}
    \ENDWHILE \\
    \STATE \textbf{return} $\argmin_{\lambda \in \Lambda} \{f(\lambda,t)\}_{(\lambda, t, f(\lambda,t)) \in H}$
  %\ENDPROCEDURE
  \end{algorithmic}
\end{algorithm}
\end{comment}

\input{icml2023/latex/algo_new}


\subsection{Prior-data Fitted Networks (PFNs)}
\label{sec:pfn}
%In this paper, we propose the use of prior-data fitted networks \citep[PFNs]{muller-iclr22a} as a dynamic surrogate model in the freeze-thaw framework (see Section~\ref{sec:ftbo}). In this section, we introduce the concept in general, the specifics of our surrogate model are described in Section~\ref{sec:surrogate}.
As briefly discussed above, PFNs~\citep{muller-iclr22a} are neural networks $q_\theta$ that are trained to do Bayesian prediction for supervised learning in a single forward pass. 
More specifically, let $D = D_{train} \cup \{(x_{test},y_{test})\}$ be a dataset used for training; the PFN's parameters $\theta$ are optimized to take $D_{train}$ and $x_{test}$ as inputs and make predictions that approximate
the posterior predictive distribution (PPD) of the output label $y_{test}$: \[q_\theta(x_{test},D_{train}) \approx Pr(y_{test}\,|\,x_{test},D_{train}),\] 
in expectation over datasets $D$ sampled from a prior $p(\mathcal{D})$ over datasets.
%\{x_i,y_i\}_{i=1}^N$ be a dataset of $N$ input-output examples. At test time, the PFN $q_\theta$ is given as input a training set $D_{train}$ and an unseen input example $x_{test}$ and outputs a discrete approximation %(Riemann distribution, see  for details)
%of the posterior predictive distribution (PPD) of the output label $y_{test}$, i.e., $q_\theta(x_{test},D_{train}) \approx Pr(y_{test}\,|\,x_{test},D_{train})$, with $(x_{test}, y_{test}) \cup D_{train} \sim p(\mathcal{D})$ the prior over datasets the PFN was fitted on. 
At test time, the PFN does not update its parameters by gradient descent given a training dataset $D_{train}$, but rather takes $D_{train}$ as a contextual input, predicting the labels of unseen examples through \emph{in-context learning}. The PFN is pretrained once for a specific prior $p(\mathcal{D})$ and used in downstream Bayesian prediction tasks without further fine-tuning. More specifically, it is trained to minimize the cross-entropy for predicting the hold-out example\textquotesingle{s} label $y_{test}$, given $x_{test}$ and $D_{train}$:
\begin{align}
\label{eq:celoss}
\begin{split}
\ell_{\theta} = \mathbb{E}[ \shortminus \text{log} \  q_{ \theta}(y_{test} |x_{test}, D_{train}) ] \\
\text{with \quad} \{(x_{test}, y_{test})\} \cup D_{train} \sim p(\mathcal{D})
\end{split}
\end{align}
\citet{muller-iclr22a} proved that this training procedure coincides with minimizing the KL divergence between the PFN\textquotesingle{s} predictions and the true PPD. 
 
%Note that PFNs are a general approach to Bayesian prediction that is widely applicable. For instance, \citet{muller-icml23} recently used PFNs as a surrogate for \emph{black-box} Bayesian optimization (\bbbo{}), where datasets are collections of hyperparameter configurations and their associated performance, i.e., $D = \{(\lambda_i, \min {f(\lambda_i,t)}_{t=1}^{b_{max}})\}_{i=1}^N$. Concurrently, \citet{adriaensen-neurips23} used PFNs as a model for Bayesian learning curve extrapolation, where datasets consisted of training time and the associated model performance for a single training run, i.e., $D = \{t,f(\lambda,t)\}_{t=1}^N$. Our method, described in next section, extends and combines both approaches, modeling performance as a function of hyperparameters, like~\citet{muller-icml23}, \emph{AND} training time, like~\citet{adriaensen-neurips23}, where datasets take the form i.e., 
 

==> icml2023/old_sections/proposed_method.tex <==


% Should probably mention these somewhere



% Problem statement:
% Given: Configuration space Lambda, validation loss, model weights after t steps of training, max training budget
% Find: Best parameter settings/model
% 
% Classical BO:
% - Evaluate configurations, training them to the max budget (one / or some initial design)
% - Fit a surrogate f(lambda): lambda --> R to this evaluation data
% - Select the next configuration as a function of the surrogate
% MF BO:
% Freeze Thaw Bayesian Optimization takes this idea to the extreme, only training for a single step
% - Train for a single step
% - Fit a surrogate f(lambda, t)
% - Acquisition policy selects what run to continue or to start a new run for some hyperparameter settings
% Unrolling 
% ==> In DPL, the surrogate took the form of a deep ensemble M(lambda)
% pseudo code
% Note that the surrogate model and acquisition function fully define the freeze-thaw method.
% In the remainder we describe these in more detail.
% lambda, t --> 
%- Surrogate
%  - PFNs
%  - prior:
%    - curve model --> show one curve example and its components, indicating the parameters
%    - bnn (not iid) --> diagram
%  - training
%  --> examples in appendix
%- Acquisition
%  --> show when which one extended
\section{In-Context Freeze-Thaw BO (\ours{})}
% Point the pseudo code difference out
In this section, we describe \ours{}, the in-context learned variant of the freeze-thaw framework that we propose as an alternative for the existing online learning implementations~\cite{wistuba-neurips22,kadra-neurips23}. As can be seen in Algorithm~\ref{algo:ftbo}, the critical difference lies in the fact that we do not need to refit our surrogate model after every allocation step, but instead provide the full history of performance observations $H$ as input for prediction. By skipping the online refitting stage, we reduce computational overhead, code complexity, and hyper-hyperparameters. Note that within the FT-BO framework described in Section~\ref{sec:ftbo}, our method is fully characterized by our choice of dynamic surrogate model (Section~\ref{sec:surrogate}) and acquisition function (Section~\ref{sec:acquisition}).


\subsection{Dynamic Surrogate Model (\ftpfn{})}
\label{sec:surrogate}
We propose \ftpfn{} a prior-data fitted network \citep[PFNs]{muller-iclr22a} trained to be used as an in-context dynamic surrogate model in the freeze-thaw framework. As described in Section~\ref{sec:pfn}, PFNs represent a general meta-learned approach to Bayesian prediction, characterized by the data used for meta-learning. % (Section \ref{sec:prior}); and the model architecture, hyperparameters, and meta-training protocol (Section \ref{sec:training}).
Following previous works using PFNs~\citep{muller-iclr22a,hollmann-iclr23,muller-icml23a,adriaensen-neurips23,dooley-neurips23}, we train the PFN only on \emph{synthetically generated data}, allowing us to generate virtually unlimited data and giving us full control over any biases therein.
We aim to train \ftpfn{} on artificial data that resembles the real performance data we observe in the context of \ftbo{}, i.e., a collection of learning curves of training runs for the same task, but using different hyperparameter settings, i.e.,
\begin{equation}
\label{eq:ftdata}
D = \{(\lambda_i,t_i), f(\lambda_i,t_i)\}_{i=1 \text{\,with\,} 1 \leq t_i \leq b_{max}}^N
\end{equation}

\paragraph{Prior desiderata:} From a Bayesian perspective, we want to generate data from a distribution that captures our prior beliefs on the relationship between hyperparameters $\lambda$, training time $t$, and model performance $f(\lambda,t)$. While one could design such prior for a specific HPO scenario, our goal here is to construct a generic prior, resulting in an \ftpfn{} surrogate for general HPO. To this end, we leverage general beliefs, e.g., we expect learning curves to be noisy, but to exhibit an improving, convex, and converging trend; curves on the same task are expected to have similar start, saturation, and convergence points; and training runs using similar hyperparameter settings to produce similar learning curves. % In what follows we describe our approach conceptually, further details can be found in Appendix~\ref{a:prior}.

% high-level: in-context LCNet
\paragraph{Prior data model:}
Following, \citet{klein-iclr17a} and \citet{kadra-neurips23}, we model the relationship between training time $t$ and $f(\lambda,t)$ by a parametric learning curve model $\hat{f}(t;\mathcal{E})$, whose parameters $\mathcal{E}$ are the output of a neural network $p(\lambda;\theta)$ taking the hyperparameter settings $\lambda$ as input (see Figure~\ref{fig:prior_model}). 
\begin{figure}
  \includegraphics[height=4cm]{icml2023/figures/ftpfn_prior.png}
  \caption{Diagram for the prior data model described in Section~\ref{sec:surrogate} that was used to generate data for meta-training \ftpfn{}. On the left, we have the randomly initialized neural network $p$ that models the relationship between a hyperparameter setting $\lambda$ and its learning curve (shown in pink), whose output parameterizes a curve model $\hat{f}$ that is a linear combination of $K$ (=2 in this illustration) basis functions (shown in red and blue) with added $\lambda$-specific Gaussian noise with variance $\sigma^2$.\label{fig:prior_model}}
\end{figure}
However, unlike these previous works, we do not train the parameters $\theta$ of this neural network. Instead, we randomly initialize the network, to represent a task-specific relationship between hyperparameters and their learning curves, which we then use to generate data for training \ftpfn{}. This can be viewed as generating samples from a Bayesian Neural Network (BNN) prior, meta-training \ftpfn{} to emulate \lcnet{}-like BNN inference through in-context learning. %, and in that sense, our approach can be viewed as emulating LCNet inference through in-context learning.
As for $p$, we adopt the same architecture and initialization procedure for the BNN prior used by \citet{muller-icml23a} in the context of \bbbo{}. The only difference here is that $p$ has $|\mathcal{E}|$ outputs, one for each parameter of our curve model $\hat{f}$, as opposed to a single output (model performance after a full training run). As for $\hat{f}$, following \citet{domhan-ijcai15a}, \citet{klein-iclr17a} and \citet{adriaensen-neurips23}, we model learning curves as a linear combination of $K$ basis functions $f_k$, with additive Gaussian noise, i.e.,
\begin{align}
\begin{split}
\hat{f}(t,\mathcal{E}) \sim \mathcal{N}(\hat{f}_{comb}(t,\mathcal{E}), {\sigma^2}) \text{\quad with} \\ 
f_{comb}(t, \mathcal{E}) = y_0 + (y_{\inf} - y_0) \cdot \sum_{k=1}^K w_k * f_k(t,\Psi_k)\\
 \text{and \quad } p(\lambda;\theta) = \mathcal{E} = \{\sigma,y_{\inf}\} \cup \{w_k\}_{k=1}^K \cup \bigcup\limits_{k=1}^{K} \Psi_{k}
\end{split}
\end{align}
where $y_0$ is the model performance after 0 training steps, and $y_{\inf}$ that at convergence.\footnote{Note that $y_0 \notin \mathcal{E}$ as we assume it to be independent of $\lambda$.} $w_k$ the weight of basis curve $f_k$, and $\Psi_k$ its the basis function specific parameters. Here, we adopt four different basis functions ($K=4$), each having four parameters, resulting in a total of 22 ($=|\mathcal{E}|$) parameters depending on $\lambda$ through $p$. Our four basis functions subsume the power law model used by~\citet{kadra-neurips23}, all three basis functions used by~\citet{adriaensen-neurips23}, and 9 of the 11 basis functions originally proposed by~\citet{domhan-ijcai15a}.\footnote{Our model excludes the two unbounded basis curves.} Furthermore, unlike those considered in previous works, our basis functions can have a breaking point~\citep{caballero-arxiv22} at which convergence stagnates or performance diverges, resulting in a more heterogeneous and realistic model.

Further details about meta-training \ftpfn{} can be found in Appendix~\ref{a:ftpfn}, including the basis curves, their parameters, and illustrations of samples from our learning curve prior (Appendix~\ref{a:lcprior}); the specific procedure we use for generating our meta-training data (Appendix~\ref{a:priorgen}); and the architecture and hyperparameters used (\ref{a:pfntraining}). 

\subsection{Dynamic Acquisition Function (\mfpirand{})}
\label{sec:acquisition}
Our dynamic acquisition function evaluates to the likelihood for every candidate configuration $\lambda \in \Lambda'$ that the model performance obtained in $h$ (\emph{horizon}) steps, will improve more than a relative \emph{threshold} $T$ upon the performance of the best model obtained thus far. Formally,
\begin{align}
\begin{split}
\text{\mfpirand}(\lambda) = \\ 
\int_{F}^{\infty} \Pr[f(\lambda, \min(t+h, b_{max}))] \, df \\
\text{with \quad} F = f_{best} + T \cdot (1-f_{best}) \\ 
\text{and \quad } f_{best} = \min {f(\lambda,t)}_{(\lambda, t, f(\lambda,t)) \in H}
\end{split}
\end{align}
Every \ftbo{} iteration both the relative threshold $T$ as the prediction horizon $h$ will be determined randomly with $h \sim \mathcal{U}(1,b_{max})$ and $log_{10}(T) \sim \mathcal{U}(-4,-1)$.

Note that existing $\ftbo{}$ implementations~\citep{wistuba-neurips22,kadra-neurips23} use Expected Improvement (EI)-based acquisition functions. However, we found these to perform poorly on some tasks, due to a lack of exploitation. In Section~\ref{sec:ablate_acquisition}, we show empirically that \ours{} indeed performs more consistently with \mfpirand{}, than when combined with EI-based acquisitions.

\iffalse
\paragraph{Motivation:} The main contribution of our paper is $\ftpfn{}$. However, to evaluate its performance in $\ftbo{}$ tasks, we must pair it with a dynamic acquisition function. Here, existing $\ftbo{}$ implementations~\citep{wistuba-neurips22,kadra-neurips23} use Expected Improvement (EI)-based acquisition functions. However, we found that this acquisition performs poorly on some tasks.
We conjecture that this failure is related to the (justified) lack of confidence $\ftpfn{}$ has about its predictions. As a result, the predicted PPD will be heavy-tailed, resulting in the high EI values for those configurations our predictions are least confident for. While this drives exploration, in the very low budget regime, this can easily lead to a failure to exploit. Our \mfpirand{} acquisition, similarly to \ei{}, will allocate resources to those configurations most likely to improve on the incumbent, more so, if this improvement is likely to be large. On the other hand, if the threshold is low, it will preferably allocate resources to configurations most likely to obtain improvements, even if they are small, i.e., exploit the sure thing, rather than explore high-risk high-gain configurations. In Section~\ref{sec:ablate_acquisition}, we show that our method indeed performs significantly better, than its EI counterparts.
\fi

\iffalse
which we then use to train and in that sense our approach is most similar to \lcnet\citep{} and can be viewed as emulating LCNet using in-context learning.

However, instead of using gradient-based MCMC methods to generate samples from the posterior, we generate 



In what follows we briefly describe our curve model, the data generation process is described in full detail in Appendix.
While this model was never used as an and it captures.
As for the BNN prior, we adopt the sampling procedure and architecture from PFNs4BO. The only difference is that instead of a single output, we have
% previous work. In particular, LC-NET
% hyperparameters --> BNN -> parameters of a learning curve model
% DPL: A similar approach, using a NN ensemble that outputs parameters of a power law curve model
% Our surrogate can be viewed as an in-context LCNET
% Meta-learned, so instead of training the , PFN learns to emulate LCNET in context.
% Benefit: online training lcnet is costly, unstable\footnote{Based our own experiences and on informal conversations with the authors and users of lcnet}

While training LCNet is unstable and 
\todo[inline]{Start with the high-level picture, contrasting with LC-NET and DPL, and LCNet}
\todo[inline]{For the rebuttal we should compare against LC-Net and against a PFN trained on the LCNet prior}



%TODO: explain high-level, contrast with LC-NET and DPL
Following, \citet{domhan-ijcai15a} and \citet{adriaensen-neurips23}, we model the performance $f$ of a model obtained after $t$ iterations of training with hyperparameter settings $\lambda$, as a linear combination of $K$ basis functions $f_k$ with added Gaussian noise with standard deviation $\sigma^\lambda$, i.e.,
\begin{align}
\begin{split}
f(\lambda, t) \sim \mathcal{N}(f_{comb}(\lambda,t), {(\sigma^\lambda)^2}) \text{\quad with} \\ 
f_{comb}(t, \lambda) = \sum_{k=1}^K w^\lambda_k * f_k(\lambda, t, \theta_k^\lambda)
\end{split}
\end{align}
where $\{w_k^\lambda\}_{k=1}^K$ are the weights of each basis curve, and $theta_k^\lambda$ the basis function specific parameters:
% Curve-specific parameters
\begin{description}
\item[$y_{0,k}^\lambda$] The initial model performance after 0 training steps.
\item[$y_{\inf,k}^\lambda$] The model performance at convergence. 
\item[$\alpha_{k}^\lambda$] The skew of the curve, affecting the convergence rate change over time in a basis-curve-specific way.
\item[$x_{sat,k}^\lambda$, $y_{sat,k}^\lambda$] The breaking point in the curve at which model performance saturates and the convergence rate is reduced with a constant factor.
\item[$r_{sat,k}^\lambda$] The reduced convergence rate after saturation, which can be negative, modeling divergence.
\end{description}
and basis function takes the form
\begin{equation}
f_k(t, \theta_k^\lambda) = f_k'(x_t,\theta_k^\lambda)
\text{with}
x_t = \frac{1}{b_{max}} \cdot \begin{cases}
        t & \text{if } t \leq x_{sat,k}^\lambda\\
        r_{sat,k}^\lambda (t - x_{sat,k}) + x_{sat,k} & \text{if } t > x_{sat,k}^\lambda
    \end{cases}
\end{equation}
a monotonic growth function $f_k$ of $x_t \in [0,1]$, which in turn is a piece-wise linear and possibly non-monotonic function of $t$, allowing us to model divergence ($r_{sat,k} < 0$), unlike prior-art~\citep{domhan-ijcai15a,adra-arxiv23a,adriaensen-neurips23}. Note that this model has many parameters, some of which are hyperparameter-specific (superscript $\lambda$) and/or basis function-specific (subscript $k$), while others are shared across hyperparameters. We construct our learning curve prior as a joint distribution over these parameters. \todo[inline]{A full table of parameters and their respective distributions can be found in Table}. It also lists the equation of the four ($K=4$) basis curves we consider that subsume the power law model by \citet{kadra-arxiv23a}, all three basis functions considered by \citet{adriaensen-neurips23}, as well as 9 of the original 11 basis functions by \citet{domhan-ijcai15a}.\footnote{\todo[inline]{Mention two basis functions that are not subsumed and motivation}}
\todo[inline]{Include a figure showing basis curves for different skews, different combinations of specific basis curves, and samples from the prior}.
\todo[inline]{Include reference to Appendix illustrating why we need > LC-PFN}.
\fi


==> icml2023/old_sections/related_work.tex <==

\section{Related Work}
\label{sec:related}

\paragraph{Multi-fidelity hyperparameter optimization} %is a popular method for optimizing expensive applications, such as training deep learning networks. This approach 
uses low-cost approximations of the objective function, for example, by evaluating only a few epochs of model training. A notable approach in this category is Hyperband~\cite{li-iclr17a}, which iteratively allocates a similar budget to various candidate hyperparameter settings and retains only the most promising ones, to be evaluated at a higher budget. Hyperband was extended for efficient parallelization~\cite{li-arxiv20a}, Bayesian optimization~\cite{falkner-icml18a} and evolutionary search~\citep{awad-ijcai21a} and to incorporate user priors~\cite{mallik2023priorband}. However, a key limitation of these multi-fidelity approaches is that they do not allow the %consider the possibility of continuing 
continuation of 
previously discarded runs in the light of new evidence, resulting in a waste of computational resources. Additionally, their effectiveness heavily depends on a good manual choice of fidelity levels and a strong correlation between the ranks of hyperparameter settings at low and high fidelities (e.g., no crossings of learning curves).

A promising research direction to mitigate these limitations involves predicting performance at higher fidelities. \citet{domhan-ijcai15a} addressed this by proposing a Bayesian learning curve extrapolation (LCE) method. Then, \citet{klein-iclr17a} extended the latter approach to jointly model learning curves and hyperparameter values with Bayesian Neural Networks. Non-Bayesian versions of LCE have also been explored by~\citet{chandrashekaran2017speeding} and ~\citet{gargiani-automl19}. Despite the robust extrapolation capabilities of these LCE methods, fully leveraging them in guiding HPO remains a challenge.

\paragraph{Freeze-Thaw Bayesian Optimization} offers a promising solution to address the limitations of standard multi-fidelity and LCE-based HPO. Its ability to pause and resume optimization runs enables the efficient management of computational resources and ensures solid anytime performance. As a BO method, it incorporates a surrogate model to predict performance at higher fidelities and relies on the acquisition function to guide the search. 
The \emph{freeze-thaw} concept was introduced by \citet{swersky-arxiv14a}, who used an entropy search acquisition function and a Gaussian Process with exponential decay kernel for modeling learning curves. \citet{wistuba-neurips22} recently proposed \dyhpo{}, an improved version that uses a learned deep kernel combined with a multi-fidelity-based Expected Improvement (EI) acquisition. Most recently, \citet{kadra-neurips23} introduced \dpl{}, another surrogate model that utilizes a deep ensemble of power laws and Expected Improvement at the maximum budget as acquisition function.
These Freeze-Thaw BO methods substantially improve upon standard multi-fidelity approaches, showing particularly strong performance in low-budget settings. Nevertheless, these methods share a common challenge: the necessity for online training of a surrogate model during the search, which can be computationally intensive and may cause optimization instabilities.


\paragraph{In-context Learning (ICL)} is an exciting new learning paradigm that offers a promising alternative to online learning methods. A key %difference and
advantage of 
%the in-context approach 
ICL 
is that it does not require retraining / fine-tuning the model with new data, but instead, the data is fed to the model as a contextual prompt.
%output of the model is conditioned on this new data by providing it as a  contextual input to the model. 
%In-context learning 
ICL 
first gained a lot of interest with the rise of Transformer-based models like Large Language Models \citep[LLMs]{radford-openaiblog19a}
%Frank: I think that is a misconception.
%, where it can be seen as a form of prompt-tuning. 
%In-context learning 
and has since also been explored 
%approach for feature engineering~\cite{hollmann-arxiv23a} and 
as an end-to-end approach to black box HPO~\cite{chen-neurips22a}. 

\paragraph{Prior data fitted networks,} proposed by \citet{muller-iclr22a}, are transformer-based models that are trained to do in-context Bayesian prediction. They have been successfully used as an in-context classifier for tabular data~\citep{hollmann-iclr23}, an in-context surrogate model for black-box HPO~\citep{muller-icml23a}, an in-context model for Bayesian learning curve extrapolation~\citep{adriaensen-neurips23}, and an in-context time-series forecaster~\citep{dooley-neurips23}. 
Our approach draws on and expands these prior works to create an efficient in-context surrogate model for freeze-thaw Bayesian Optimization.
%Our approach seeks to combine PFNs4BO~\citep{muller-icml23a} and LC-PFN~\citep{adriaensen-neurips23}, creating an efficient in-context surrogate model for freeze-thaw Bayesian Optimization. %The motivation of our work is to tackle issues of existing online learning based approaches such as DPL and DyHPO. To our knowledge, no prior works have proposed a combination of BO with learning curve extrapolation within an in-context approach.

\begin{comment}
    

\paragraph{Multi-fidelity Hyperparameter Optimization:}
    \begin{itemize}
    \item Hyperband~\citep{li-iclr17a} and extensions (ASHA~\citep{li-mlsys20a}, BOHB~\citep{falkner-icml18a}, Mobster~\citep{klein-arxiv20a}, DEHB~\citep{awad-ijcai21a}, iterative deepening HB~\citep{brandt-arxiv23})
    \item Is a single epoch all you need?~\citep{egele-arxiv23}
    \item HPO with Learning curve extrapolation (cite the survey here!): 
    \begin{itemize}
        \item Bayesian: LC-NET~\citep{klein-iclr17a}
        \item Non-Bayesian~\citep{chandrashekaran2017speeding,gargiani-automl19}
    \end{itemize}
    \item Dynamic / Freeze-Thaw style HPO: 
    \begin{itemize}
    \item Freeze-Thaw~\citep{swersky-arxiv14a}
    \item DyHPO~\citep{wistuba-neurips22}
    \item DPL~\citep{kadra-arxiv23a}
    \end{itemize}
\end{itemize}
\paragraph{In-context Learning and PFNs}
\begin{itemize}
    \item Other work using in-context learning (LLMs), in particular in the AutoML realm?
    \item Neural processes!
    \item Previous work using PFNs. In particular, LC-PFN~\citep{adriaensen-neurips23} and PFNs4BO~\citep{muller-icml23}
    \item MASIF~\citep{ruhkopf-tmlr22} (similar: input, transformer, in-context learning; different: output (rank at end of training), non-Bayesian, no acquisition policy, trained for a specific algorithm space)
\end{itemize}

\end{comment}

==> icml2023/sections/surrogate_model_rebu.tex <==
\subsection{Dynamic Surrogate Model (\ftpfn{})}
\label{sec:surrogate}
We propose \ftpfn{} a prior-data fitted network \citep[PFNs]{muller-iclr22a} trained to be used as an in-context dynamic surrogate model in the freeze-thaw framework. As described in Section~\ref{sec:pfn}, PFNs represent a general meta-learned approach to Bayesian prediction, characterized by the data used for meta-training. % (Section \ref{sec:prior}); and the model architecture, hyperparameters, and meta-training protocol (Section \ref{sec:training}).
Following previous works using PFNs~\citep{muller-iclr22a,hollmann-iclr23a,muller-icml23a,adriaensen-neurips23,dooley-neurips23}, we train the PFN only on \emph{synthetically generated data}, allowing us to generate virtually unlimited data and giving us full control over any biases therein.
We aim to train \ftpfn{} on artificial data ($D$) that resembles the real performance data we observe in the context of freeze-thaw Bayesian optimization, i.e., a collection of learning curves of training runs for the same task, but using different hyperparameter settings, i.e., $\bigcup_{\lambda\in\Lambda}\{(\lambda,z_i), \loss(\lambda,z_i \cdot \mathds{1}_b)\}_{i=1}^{b_{\text{max}}}$. To reduce the entropy of this prior (and PFN training time), we assume this data to be normalized. In particular
%\begin{comment}
% \begin{equation}
% % \tiny
% \label{eq:ftdata}
% % \editmode{
% D = \bigcup_{\lambda\in\Lambda}\{(\lambda,t_i), f(\lambda,t_i)\}_{i=1}^{b_{\text{max}}} 
% \sim \bigcup_{\lambda\in\Lambda}\{(\lambda,\frac{z_i}{b_{\text{max}}}), \frac{\loss(\lambda,\frac{z_i}{b_{\text{max}}} \cdot \mathds{1}_b)}{\loss_{\text{max}}-\loss_{\text{min}}}\}_{i=1}^{b_{\text{max}}}
% % }
% \end{equation}


\begin{equation}
    \centering
    \label{eq:ftdata}
    \begin{gathered}
        D = \bigcup_{\lambda\in\Lambda}\left\{(\lambda,t_i), f(\lambda,t_i)\right\}_{i=1}^{b_{\text{max}}} \\
        D \sim \bigcup_{\lambda\in\Lambda}\left\{\left(\lambda,\frac{z_i}{b_{\text{max}}}\right), \frac{\loss(\lambda,\frac{z_i}{b_{\text{max}}} \cdot \mathds{1}_b)}{\loss_{\text{max}}-\loss_{\text{min}}}\right\}_{i=1}^{b_{\text{max}}}
    \end{gathered}
\end{equation}

\editmode{
Note that since $\mathds{1}_b$ acts as a constant scaling factor, and we will normalize $z_i$ w.r.t. $b_{\text{max}}$, we consider $\{(\lambda_i,t_i), f(\lambda_i,t_i)\}_{i=1 \text{\,with\,} 0 \leq t_i \leq 1}^N$ as dataset when discussing our surrogate.
}
\neeratyoy{In our setup, $f_{\text{max}}=1$ and $f_{\text{min}}=0$.}

\paragraph{Prior desiderata:} From a Bayesian perspective, we want to generate data from a distribution that captures our prior beliefs on the relationship between hyperparameters $\lambda$, training time $t$, and model performance $f(\lambda,t)$. While one could design such prior for a specific HPO scenario, our goal here is to construct a generic prior, resulting in an \ftpfn{} surrogate for general HPO. To this end, we leverage general beliefs, e.g., we expect learning curves to be noisy, but to exhibit an improving, convex, and converging trend; curves on the same task are expected to have similar start, saturation, and convergence points; and training runs using similar hyperparameter settings to produce similar learning curves. % In what follows we describe our approach conceptually, further details can be found in Appendix~\ref{a:prior}.

% high-level: in-context LCNet
\paragraph{Prior data model:}
Following, \citet{klein-iclr17a} and \citet{kadra-neurips23}, we model the relationship between training time $t$ and $f(\lambda,t)$ by a parametric learning curve model $\hat{f}(t;\mathcal{E})$, whose parameters $\mathcal{E}$ are the output of a neural network $p(\lambda;\theta)$ taking the hyperparameter settings $\lambda$ as input (see Figure~\ref{fig:prior_model}). 
\begin{figure}
  \includegraphics[height=4cm]{icml2023/figures/ftpfn_prior.png}
  \caption{Diagram for the prior data model described in Section~\ref{sec:surrogate} that was used to generate data for meta-training \ftpfn{}. On the left, we have the randomly initialized neural network $p$ that models the relationship between a hyperparameter setting $\lambda$ and its learning curve (shown in pink), whose output parameterizes a curve model $\hat{f}$ that is a linear combination of $K$ (=2 in this illustration) basis functions (shown in red and blue) with added $\lambda$-specific Gaussian noise with variance $\sigma^2$.\label{fig:prior_model}}
\end{figure}
However, unlike these previous works, we do not train the parameters $\theta$ of this neural network. Instead, we randomly initialize the network, to represent a task-specific relationship between hyperparameters and their learning curves, which we then use to generate data for training \ftpfn{}. This can be viewed as generating samples from a Bayesian Neural Network (BNN) prior, meta-training \ftpfn{} to emulate \lcnet{}-like~\citep{klein-iclr17a} BNN inference through in-context learning. %, and in that sense, our approach can be viewed as emulating LCNet inference through in-context learning.
As for $p$, we adopt the same architecture and initialization procedure for the BNN prior used by \citet{muller-icml23a} in the context of black box BO. The only difference here is that $p$ has $|\mathcal{E}|$ outputs, one for each parameter of our curve model $\hat{f}$, as opposed to a single output (model performance after a full training run). As for $\hat{f}$, following \citet{domhan-ijcai15a}, \citet{klein-iclr17a} and \citet{adriaensen-neurips23}, we model learning curves as a linear combination of $K$ basis functions $f_k$, with additive Gaussian noise, i.e.,
\begin{align}
\begin{split}
\hat{f}(t,\mathcal{E}) \sim \mathcal{N}\left(\hat{f}_{comb}(t,\mathcal{E}), {\sigma^2}\right) \text{\quad with} \\ 
f_{comb}(t, \mathcal{E}) = y_0 + (y_{\infty} - y_0) \cdot \sum_{k=1}^K w_k f_k(t,\Psi_k)\\
 \text{and \quad } 
 \editmode{p(\lambda;\theta) = \mathcal{E} = \left(\sigma,y_{\infty},w_1,\ldots, w_K, \Psi_{1},\ldots,\Psi_K\right)}
\end{split}
\end{align}
% \todo{add unifying equation/text - steven: having thought about it we cannot add a M = LC-PFN equation here as this is the training data of the PFN - not inference}
where $y_0$ is the model performance after 0 training steps, and $y_{\infty}$ that at convergence.\footnote{Note that $y_0 \notin \mathcal{E}$ as we assume it to be independent of $\lambda$.} $w_k$ the weight of basis curve $f_k$, and $\Psi_k$ its the basis function specific parameters. Here, we adopt four different basis functions ($K=4$), each having four parameters, resulting in a total of 22 ($=|\mathcal{E}|$) parameters depending on $\lambda$ through $p$. Our four basis functions subsume the power law model used by~\citet{kadra-neurips23}, all three basis functions used by~\citet{adriaensen-neurips23}, and 9 of the 11 basis functions originally proposed by~\citet{domhan-ijcai15a}.\footnote{Our model excludes the two unbounded basis curves.} Furthermore, unlike those considered in previous works, our basis functions can have a breaking point~\citep{caballero-iclr23} at which convergence stagnates or performance diverges, resulting in a more heterogeneous and realistic model.

Further details about meta-training \ftpfn{} can be found in Appendix~\ref{a:ftpfn}, including the basis curves, their parameters, and illustrations of samples from our learning curve prior (Appendix~\ref{a:lcprior}); the specific procedure we use for generating our meta-training data (Appendix~\ref{a:priorgen}); and the architecture and hyperparameters used (\ref{a:pfntraining}). 
